Inference without Interference: Disaggregate LLM Inference for Mixed Downstream Workloads

Transformer-based large language model (LLM) inference serving is now the backbone of many cloud services. LLM inference consists of a prefill phase and a decode phase. However, existing LLM deployment practices often overlook the distinct characteristics of these phases, leading to significant interference. To mitigate interference, our insight is to carefully schedule and group inference requests based on their characteristics. We realize this idea in TetriInfer through three pillars. First, it partitions prompts into fixed-size chunks so that the accelerator always runs close to its computationsaturated limit. Second, it disaggregates prefill and decode instances so each can run independently. Finally, it uses a smart two-level scheduling algorithm augmented with predicted resource usage to avoid decode scheduling hotspots. Results show that TetriInfer improves time-to-first-token (TTFT), job completion time (JCT), and inference efficiency in turns of performance per dollar by a large margin, e.g., it uses 38% less resources all the while lowering average TTFT and average JCT by 97% and 47%, respectively.

==> fig-dfv-p-layer-qos.tex <==
{
\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=0.4\textwidth]{Figures/dfv-p-layer-qos.pdf}}
\mycaption{fig-p-layer-qos}{Isolation and QoS in the Persistence Layer.}
{
}
\end{center}
\end{figure}
}

==> fig-prefill-dispatcher.tex <==
{
\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=0.47\textwidth]{Figures/fig_prefill_dispatcher.pdf}}
\caption{\textbf{Prefill Instance Dispatcher Workflow.}}
\label{fig-prefill-dispatcher}
\end{center}
\end{figure}
}

==> fig-prefill-scheduler-compare.tex <==

{
\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=0.47\textwidth]{Figures/fig_benfits_of_chuned_prefill_scheduler_policy.pdf}}
\caption{\textbf{Scheduler Policies and Chunked Prefill.} Both figures show TTFT's CDF. Higher the better.}
\label{fig-prefill-scheduler-compare}
\end{center}
\end{figure}
}

==> note.tex <==
\section{Note}

This section is for notes, it is not part of the paper.

\begin{itemize}
    \item  \Q{Some companies chose FS semantics such as GFS Colossus, Tectonic; some chose append-only semantic such as DFV, WAS. What's the trade-off here?} \A{ (1) from a technical point of a view, FS requires extensive metadata management, and consequently its consistency and fault-tolerance. So a DFS abstraction will be more complex than a pure append-only abstraction. Then, the question falls back to, do all services running on top of DFV build their own metadata manegement layer? If so, is it better to have it in the P layer? We need good answers.}
    
\item
\Q{What services are not a good fit to build on top of DFV, the append-only semantic?}

\item
\Q{Merits of Plog}
\A{(1) Check out the Taurus paper section 3.3. The insight I found is that failure is not transparently handled by the lowest-layer software such as P-layer, but rather exposed to the applications. Fast fail over. This design philosophy was used by several notable networking projects and others.
(2) good for SSDs, wear-leveling etc. (3) comparison to a FS interface, no overuse of metadata.}

\end{itemize}


==> tbl-categorization.tex <==
\begin{table}\scriptsize
    \centering
    \begin{tabular}{ | c | c | c | c | c |}
    \hline
        & \textbf{\HP} & \textbf{\LP} &  \textbf{\HD} & \textbf{\LD} \\
    \hline
      \textbf{ \HP} & \S\ref{sec-bg-pp}  &    &  & \\
    \hline
       \textbf{\LP} & \S\ref{sec-bg-pp}  & \S\ref{sec-bg-pp} & & \\
    \hline
       \textbf{\HD} & \S\ref{sec-bg-pd}   & \S\ref{sec-bg-pd}  & \S\ref{sec-bg-dd}& \\
    \hline
       \textbf{\LD} &  \S\ref{sec-bg-pd}   & \S\ref{sec-bg-pd}  & \S\ref{sec-bg-dd} & \S\ref{sec-bg-dd} \\
    \hline
    \end{tabular}
    \caption{\textbf{Inferecen Task Combinations}. A cell means running two types of requests together, e.g., heavy prefill and heavy prefill in the same batch. Content refers to sections.}
    \label{table-categorization}
\end{table}

==> tbl-configuration.tex <==

\begin{table}
    \centering
    \begin{tabular}{ | p{0.8in} | p{0.8in} | c |  }
    \hline
       Model size & 13B & 125M  \\
    \hline
       GPUs   &  V100       &  \\
    \hline
       GPU Memory &  32 GB   &  \\
    \hline
       Parameter size &  25.8GB  & 0.3GB \\
    \hline
    \end{tabular}
    \caption{\textbf{Model sizes and configuration for \sysname.}}
    \label{table-configuration}
\end{table}


==> tbl-deployment.tex <==

\begin{table}
    \centering
    \begin{tabular}{ | p{0.8in} | c | c | }
    \hline
       Option & Dispatch KV & Description \\
    \hline
       Co-located   &  N/A       & 3 \\
    \hline
       Intra-Server &  via-CPU   & 3 \\
    \hline
       Intra-Server &  Direct  & 3 \\
    \hline
       Inter-Server &  via NIC & 3 \\
    \hline
       Inter-Server &  Direct & 2  \\
    \hline
    \end{tabular}
    \caption{\textbf{Hardware deployment options for \sysname.}}
    \label{table-deployment}
\end{table}

==> tbl-predict-accuracy.tex <==

\begin{table}
    \centering
    \begin{tabular}{ | p{0.8in} | p{0.8in} | c |  }
    \hline
       Work & Alpaca & ShareGPT  \\
    \hline
       S3   &  98.61\%       &  \\
    \hline
       Seq-Sched &  81\%   &  \\
    \hline
       \sysname\ &  82.9\%  & 74.9\% \\
    \hline
    \end{tabular}
    \caption{\textbf{Predict Model' s accuracy. acc-100. }}
    \label{table-predcit-accuracy}
\end{table}
